NoScope: Optimizing Neural Network Queries over Video at Scale

Recent advances in computer vision-in the form of deep neural networks-have made it possible to query increasing volumes of video data with high accuracy. However, neural network inference is computationally expensive at scale: applying a state-of-the-art object detector in real time (i.e., 30+ frames per second) to a single video requires a $4000 GPU. In response, we present NoScope, a system for querying videos that can reduce the cost of neural network video analysis by up to three orders of magnitude via inference-optimized model search. Given a target video, object to detect, and reference neural network, NoScope automatically searches for and trains a sequence, or cascade, of models that preserves the accuracy of the reference network but is specialized to the target video and are therefore far less computationally expensive. NoScope cascades two types of models: specialized models that forego the full generality of the reference model but faithfully mimic its behavior for the target video and object; and difference detectors that highlight temporal differences across frames. We show that the optimal cascade architecture differs across videos and objects, so NoScope uses an efficient cost-based optimizer to search across models and cascades. With this approach, NoScope achieves two to three order of magnitude speed-ups (265-15,500x real-time) on binary classification tasks over fixed-angle webcam and surveillance video while maintaining accuracy within 1-5% of state-of-the-art neural networks.

==> demo.tex <==
\section{Demonstration}

\begin{comment}

- At SIGMOD we will present an end-to-end demo of VUSE, which will consist of
two parts: 1) we will allow users to semantically queries a large stored video
dataset, 2) we will demonstrate the effect of cascades of filters through live
video streams, demonstrating that VUSE can index video in real time.

- We will focus the stored dataset on people: users can ask queries such as
"when did people leave the office" and "what was the most number of people in
the office"
-- Mention data sets. The public ones seems fairly short, so maybe we will have
to make our own?
-- Talk about the interface (what should this look like?  Database queries or
NLP?)

- The live demo will allow users to select and order the cascade of filters,
which will demonstrate how the cascade of filters affects performance.
Additionally, we will index the streams in real-time and allow queries to the
stored video.
-- Live streams of SIGMOD or webcams we set up elsewhere (e.g.  back at
Stanford), or have VUSE index stored video in real-time?
-- Mentioned some possible queries. How many people entered the scene up until
now?

\end{comment}

At SIGMOD, we will present an end-to-end demonstration of \vuse
that illustrates both the value of a high-level query interface for
video as well as the importance of dynamic model cascades.

\minihead{Datasets and queries} We plan to run \vuse over live video
to collect statistics about the SIGMOD demonstration room. That is, we
will deploy a small set of webcams in and around the SIGMOD conference
to enable users to answer queries including: ``how many people have
visited the VUSE demo?''; ``what fraction of SIGMOD attendees entering
the demo room attended the VUSE demo?''; and ``what fraction of demo
attendees' time is spent at the VUSE demo?'' (One concern for the demo
PC may be that the answer to the latter question may in fact be quite
high, although we will be happy to provide all statistics to the
demo judges.) We will also allow attendees to issue queries over a
range of live video streams, including both open webcams on the public
Internet as well as streaming video sites including Twitch and
Periscope. Our development plans for summer 2017 include a public
website for performing the latter class of queries, so SIGMOD
attendees will be subject to an early sneak peek.

For the latter class of external Internet video streams, to enable
users to query the streams ingested by \vuse, we will provide conference
attendees with a web user interface that allows them to select 1) the
video streams to query, 2) the semantic query. Once the video stream
and query are selected, they will be processed and \vuse will present
the results along with relevant parts of the video stream. For
example, for the query "which demo currently has the most
attendees?", \vuse will show the part of the video feed with
that demo. Users can also optionally ask \vuse to label images
in the frame to see how the CNN labels them.

%\begin{figure}[ht!]
%  \includegraphics[width=0.97\textwidth]{figures/filter_selection_ui_FIXME.png}
%  \caption{The UI for users to select and order filter cascades.
%    After the user prepares the cascade, a view of what the filter
%    ``sees'' is presented.}
%  \label{fig:ui_filters}
%\end{figure}

\minihead{Demonstrating the effect of cascades} As each model focuses on a
particular aspect of the video stream, we will prepare live visualizations of
how the models ``see" the video. Our goal is to show how individual models
interact with each individual frame of  an entire video clip. Therefore, in our
interface, end-users will be able to watch videos and see what each of our
models sees in real-time.  For example, to visualize the effects of the color
histogram model, we will display the color histograms of the frames being
analyzed and the corresponding $\chi^2$ value.

Additionally, to demonstrate the performance improvements for the models, we
will indicate the time spent on each model and the estimated time if the CNN
were run on every frame. We will also provide a separate interface, which
attendees will also interact with via the web, to explore the impact of
ordering in the model cascade. Figure \ref{fig:vuse_diagram} gives an example
of such an ordering using the models enumerated in Section \ref{sec:filters};
our interface will enable users to toggle each model on or off (e.g. deactivate
Simple Skipping), as well as re-order models (e.g. swap the order of Background
Subtraction and Color Histogram) to change the sequence in which they are
applied to each frame.  Once the model cascade has been configured by the user,
our interface will provide a benchmark comparison of the efficiency and
accuracy of these changes on the available datasets. This enables the
attendees to explore the performance impact of our dynamic model
cascade at fine granularity: per model, per ordering, and per video
stream.

\begin{comment}
Our demonstration will consist of a web user interface that allows users to
directly query the \vuse system on a variety of public video datasets, including
the \todo{insert datasets here}. In addition, we will provide video streams that
we've collected on our own; together, these video streams capture a wide variety
of foreground and background scenes that \vuse will index. Upon issuing a query,
users will then view which frames from which video streams contain the object
classes that match the query; we explain the query semantics interface in the
following section. Furthermore, we will also provide an interface that allows
users to explore the impact of key optimizations implemented in \vuse across the
different datasets.  Lastly, we will provide a webcam during our demo; users
will be able to query for different object classes that are present in the video
feed from the webcam and see the results in real time.

\subsection{VUSE Query Interface}
To enable users to query the videos indexed by \vuse, we will provide
conference attendees with a web user interface that allows them to select 1)
the video streams to query, and 2) the object classes to detect within each
video stream. Users will first be asked to select a video to query---they can
do this by clicking on the video thumbnail (Figure \ref{fig:ui_video}). Next,
for that particular video, our user interface will present a list of possible
object classes to search for; users will be asked to select at least one object
class using a checkbox interface (Figure \ref{fig:ui_classes}). Users can
repeat this process for as many videos as they wish; once the query has been
prepared and submitted, \vuse will then present the results for each video as a
series of still frames: each frame will be identified by its timestamp, with
the relevant object classes in the frame labeled with colored bounding boxes
(Figure \ref{ui_results}).  This same interface will be used for interactively
querying the live video stream from the webcam.

\subsection{Exploring Impact of Frame Filtration}
Additionally, to demonstrate the efficacy of our frame filtration
optimizations, we will also provide an opportunity for conference attendees to
manipulate filters on a single video stream and see the resulting impact on
query performance.

\end{comment}

